Improving Joint Training of Inference Networks and Structured Prediction Energy Networks

Deep energy-based models are powerful, but pose challenges for learning and inference (Belanger and McCallum, 2016). Tu and Gimpel (2018) developed an efficient framework for energy-based models by training "inference networks" to approximate structured inference instead of using gradient descent. However, their alternating optimization approach suffers from instabilities during training, requiring additional loss terms and careful hyperparameter tuning. In this paper, we contribute several strategies to stabilize and improve this joint training of energy functions and inference networks for structured prediction. We design a compound objective to jointly train both cost-augmented and test-time inference networks along with the energy function. We propose joint parameterizations for the inference networks that encourage them to capture complementary functionality during learning. We empirically validate our strategies on two sequence labeling tasks, showing easier paths to strong performance than prior work, as well as further improvements with global energy terms.

==> analysis.tex <==
\section{Qualitative Analysis}


As shown in Table \ref{table:phi-vs-psi}, our compound objective with joint training of the cost-augmented and test-time inference networks yields larger differences in performance between the two inference networks. In this section, we analyze how the two differ. 
%to show these differences between $\infnet$ and $\canet$, exploring the different patterns of these two inference networks.

%Given the trained $\canet$ and $\infnet$, 
On the POS development set, we count the differences between the predictions of $\infnet$ and $\canet$ in cases where $\infnet$ makes the correct prediction. For this we used the BiLSTM version of the stacked parameterization. % (BiLSTM). 
The top 10 most frequent prediction pairs are shown in Table \ref{table:qa}. The most frequent combinations show that $\canet$ tends to output tags that are highly confusable with those output by $\infnet$. For example, it often outputs proper noun when the gold standard is common noun or vice versa. It also captures the noun-verb ambiguity and ambiguities among adverbs, adjectives, and prepositions. 

\begin{table}[t]
\small
\begin{center}
\begin{tabular}{cc}
test-time ($\infnet$)  & cost-augmented ($\canet$) \\% & $\infnet$ & $\canet$  \\
\hline
 common noun  & proper noun \\
 proper noun & common noun   \\
 common noun  & adjective  \\
 proper noun  & proper noun + possessive\\
 adverb & adjective \\
 preposition & adverb \\
 adverb & preposition \\
 verb &  common noun\\
 adjective & verb \\
 common noun &  verb \\
%, & 96.7 & E  &$\wedge$ & 71.7 &A \\
\end{tabular}
\end{center}
\caption{Top 10 most frequent output differences between $\infnet$ and $\canet$. \lifu{Move to appendix}
%\kevin{fix this caption; accuracy rates are not shown anymore. also please define the tags (people won't know what they stand for) or else use longer tag names in the table like ``noun'', ``proper noun'', etc.}\lifu{I see}
}\label{table:qa}
\end{table}


==> contribs.tex <==
\begin{itemize}
    \item We use multi-task learning to jointly train both cost-augmented and test-time inference networks along with the energy function. 
    \item We propose shared parameterizations for the two inference networks   that   encourage   them   to   capture complementary  functionality  while reducing the number of parameters being trained 
    \item We propose three simple methods to streamline and stabilize training with the above objective
    \item We empirically validate our strategies on two sequence labeling tasks, showing easier paths to strong performance than prior work, and further  improvements  with  global  energy terms
\end{itemize}

